Characterization of Market Models in the Presence of Traded Vanilla and Barrier Options

We characterize the set of market models when there are a finite number of traded Vanilla and Barrier options with maturity $T$ written on the asset $S$. From a probabilistic perspective, our result describes the set of joint distributions for $(S_T, \sup_{u \leq T} S_u)$ when a finite number of marginal law constraints on both $S_T$ and $\sup_{u \leq T} S_u$ is imposed. An extension to the case of multiple maturities is obtained. Our characterization requires a decomposition of the call price function and once it is obtained, we can explicitly express certain joint probabilities in this model. In order to obtain a fully specified joint distribution we discuss interpolation methods.

==> arbitrage.tex <==

\section{Arbitrage}
\label{sec:arbitrage}

In this section we investigate what types of arbitrage arise if the conditions of Theorem \ref{thm:Characterization Market Model - Multiple Maturity} fail.
\begin{Proposition}[Arbitrage]
\label{prop:arbitrage}
Let Assumption \ref{ass:asset and market} hold. 
Assume that there is no weak arbitrage in the call prices\footnote{i.e. amongst others, $c_{\mu_l}(K_i)>c_{\mu_l}(K_{i+1})$ for $K_i < K_{i+1}$ and $c_{\mu_l}(K) \to 0$ as $K \to \infty$.}, i.e. $c_{\mu_l}(\cdot) = \int (y-\cdot)^+ \mu_l( \dd y )$ for a probability measure supported on $\R_+$ with a finite mean. 

Then, there is no market model if and only if for all $N>0$ there exist constants $\lambda^{\mathrm{V}}_{i,l}, \lambda^{\mathrm{B}}_{j,l}$ such that 
\begin{alignat}{3}
& && &&\sum_{l=1}^k \left( \sum_{i=1}^{n} \lambda_{i,l}^{\mathrm{V}} \cdot c_l(K_i) + \sum_{j=1}^{m} \lambda_{j,l}^{\mathrm{B}} \cdot b_l(B_j) \right) \nonumber \\
>& \sup_{\boldsymbol{\tau} \in \mathcal{T}^N } 
&&\EE_{\PP_0} \Bigg[ &&\sum_{l=1}^{k} \left( \sum_{i=1}^{n} \lambda_{i,l}^{\mathrm{V}} \cdot \left( X_{\tau_l} - K_i \right)^+ + \sum_{j=1}^{m} \lambda_{j,l}^{\mathrm{B}} \cdot \indicator{ M_{\tau_l} \geq B_j } \right) \Bigg] \label{eq:arbitrage} \\
=& \hspace{1mm} \sup_{ \PP } 
&&\EE_{\PP} \Bigg[ &&\sum_{l=1}^{k} \left( \sum_{i=1}^{n} \lambda_{i,l}^{\mathrm{V}} \cdot \left( S_{T_l} - K_i \right)^+ + \sum_{j=1}^{m} \lambda_{j,l}^{\mathrm{B}} \cdot \indicator{ M_{T_l} \geq B_j } \right) \Bigg]
\nonumber
\end{alignat}
where $X$ is a $\PP_0$-Brownian motion, $X_0 = S_0$, 
\begin{align*}
\mathcal{T}^N := \left\{ (\tau_1, \dots, \tau_k ) \in \mathcal{T}_{\infty}^k : \tau_1 \leq \dots \leq \tau_k \leq H_{N} \right\}
\end{align*}
and the second supremum is over all martingale measures $\PP$ satisfying $\Prob{ S_{T_l} > N } = 0$.
\end{Proposition}

\begin{Remark}[Realizing the Arbitrage]
Choose an arbitrary $N<\infty$. 
Proposition \ref{prop:arbitrage} suggests that an arbitrage can be realized if $M_T \leq N$ by selling the payoff 
\begin{align}
\sum_{l=1}^k \left( \sum_{i=1}^{n} \lambda_{i,l}^{\mathrm{V}} \cdot \left( S_{T_l} - K_i \right)^+ + \sum_{j=1}^{m} \lambda_{j,l}^{\mathrm{B}} \cdot \indicator{ M_{T_l} \geq B_j } \right)
\label{eq:to_be_superreplicated}
\end{align}
for its market price
\begin{align*}
\sum_{l=1}^k \left( \sum_{i=1}^{n} \lambda_{i,l}^{\mathrm{V}} \cdot c_l(K_i) + \sum_{j=1}^{m} \lambda_{j,l}^{\mathrm{B}} \cdot b_l(B_j) \right)
\end{align*}
and superreplicating\footnote{It remains to be investigated whether the superreplicating strategy for \eqref{eq:to_be_superreplicated} exists in pathwise sense or only in quasi-sure sense.} -- under the premise that $M_T \leq N$ -- for a strictly smaller cost.

We also note that this suggests that, in general, the arbitrage will be realized by dynamically trading in the underlying and not by a static portfolio only.
\end{Remark} 

\begin{proof}[Proof of Proposition \ref{prop:arbitrage}]
The second equality in \eqref{eq:arbitrage} holds by the Dambis-Dubins-Schwarz time change.

Recall from Theorem \ref{thm:Characterization Market Model - Multiple Maturity} that there exists a market model if and only if there exists a market model with upper  bound of support $N$. 
Define the compact set
\begin{align*}
\mathcal{K} = \Bigg\{ \left\{ c^{B_j}_{l} \right\}_{ l,j } \hspace{1mm} : \hspace{2mm} &\text{\eqref{eq:cond_a} -- \eqref{eq:cond_e} holds for some }   \\
  &\text{call price functions $c_{\mu_l}$, $c_{\mu_l}(K)=0$ for $K \geq N$,} \\
  &\text{and some barrier prices $\bb_l$}  \Bigg\}.
\end{align*}
It follows from Theorem \ref{thm:Characterization Market Model - Multiple Maturity} that we can identify each element $\boldsymbol{\tau} \in \mathcal{T}^N$ with one element in $\mathcal{K}$.
Therefore, the claim is a reformulation of \citet[Theorem 1]{fan57}, which we recall for the readers convenience in the appendix \ref{app:fan_existence_thms}.
\end{proof}

 

 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
\begin{comment}

\begin{align*}
&\sup_{\tau \in \mathcal{T}^{\star}_{\infty}} \E{ 0 } \\
=&\sup_{\tau \in \mathcal{T}_{\infty}} \inf_{\bl^{\mathrm{V}}, \bl^{\mathrm{B}}}  \E{ 0 - \sum_{i=1}^{n^{\mathrm{V}}} \lambda_i^{\mathrm{V}} \left( X_{\tau} - K_i \right)^+ - \sum_{j=1}^{n^{\mathrm{B}}} \lambda_j^{\mathrm{B}} \indicator{ M_{\tau} \geq B_j } } + 
\sum_{i=1}^{n^{\mathrm{V}}} \lambda_i^{\mathrm{V}} c_{K_i} + \sum_{j=1}^{n^{\mathrm{B}}}  \lambda_j^{\mathrm{B}} b_{B_j} \\
=&\inf_{\bl^{\mathrm{V}}, \bl^{\mathrm{B}}} \sup_{\tau \in \mathcal{T}_{\infty}} \E{ 0 - \sum_{i=1}^{n^{\mathrm{V}}} \lambda_i^{\mathrm{V}} \left( X_{\tau} - K_i \right)^+ - \sum_{j=1}^{n^{\mathrm{B}}} \lambda_j^{\mathrm{B}} \indicator{ M_{\tau} \geq B_j } } + 
\sum_{i=1}^{n^{\mathrm{V}}} \lambda_i^{\mathrm{V}} c_{K_i} + \sum_{j=1}^{n^{\mathrm{B}}}  \lambda_j^{\mathrm{B}} b_{B_j} \\
=&\inf\left\{ V_0: \exists \phi, \bl^{\mathrm{V}}, \bl^{\mathrm{B}} \text{ s.t. } V_0 + (\phi \cdot X)_t + 
\sum_{i=1}^{n^{\mathrm{V}}} \lambda_i^{\mathrm{V}} \left( \left( X_{t} - K_i \right)^+ - c_{K_i} \right) \right. \nonumber \\
&\left. \hspace{3.5cm}+ \sum_{j=1}^{n^{\mathrm{B}}} \lambda_j^{\mathrm{B}} \left( \indicator{ M_{t} \geq B_j } - b_{B_j}  \right) \geq 0 \text{ a.s. for all $t \in \R_+$ } \right\} 
\end{align*}
where by the usual convention
\begin{align}
\sup_{\tau \in \mathcal{T}^{\star}_{\infty}} \E{ 0 } = 
\begin{cases} 0 &\mbox{if } \mathcal{T}_{\infty}^{\star} \neq \emptyset \\
-\infty & \mbox{else. }  \end{cases} 
\end{align} 

\end{comment} 

==> construction_of_models.tex <==

\section{Construction of Market Models}
\label{sec:Construction of Calibrated Models}

Next we show how one can obtain market models more explicitly.

In the context of only traded Vanilla options, \citet{CarrGamma} argues that subordinated diffusion processes are models with desirable properties.
Hence, one might argue that in our context of both, traded Vanilla and Barrier options, a suitable extension will yield a \enquote{reasonable} model.
This extension has been obtained by \citet{RePEc:eee:spapps:v:121:y:2011:i:12:p:2802-2817} who constructs a Gamma subordinated diffusion-type process under some regularity conditions.

In the case of multiple maturities, we formally show how to obtain a generalized Dupire formula.
A more rigorous account for these arguments is reported by \citet{Forde13} and \citet{Forde14} who derive a generalized forward Kolmogorov equation and specify a calibrated diffusion-type process under some regularity assumptions.


\subsection{Gamma Subordinated Diffusion-Type Process for one Maturity}

Recall the definition of $\mathcal{M}_T$ from section \ref{subsec:Interpolation of Barrier Prices}.
We assume that $\mathcal{M}_T$ has a bounded, continuous and strictly positive density $f_T$ on
\begin{align*}
\big\{ (x,m) \in \R^2 \ : \ x \leq m, \ X_0 \leq m \big\}.
\end{align*}
 
%\begin{align}
%f_T(x,m) := \frac{ \Prob{ X_{\tau_T} \in \dd x, M_{\tau_T} \in \dd m }}{\dd x \dd m}
%\end{align}

Define
\begin{align}
\sigma^2(x,m) := \frac{ 2 \lambda \int_{-\infty}^{\infty} ( x-y )^+ f_T(y,m) \dd y }{f_T( x,m )}  
\end{align}
for $x \leq m$ and $\lambda > 0$.

Under some conditions on $\sigma$, \citet[Proposition 3.2]{RePEc:eee:spapps:v:121:y:2011:i:12:p:2802-2817} constructs
a non-exploding weak solution to the Stochastic Functional Differential Equation (SFDE) 
\begin{align}
Y_t = Y_0 + \int_0^t \sigma(Y_u,M_u) \dd W_u.
\end{align}

Following \citet{CarrGamma}, let $(\Gamma_t)_{t>0}$ be an independent gamma process with \Levy density $k_{\Gamma}(t) = \frac{e^{-\frac{t}{T}}}{T \cdot t}, t>0$.


Then \citet[Proposition 5.2]{RePEc:eee:spapps:v:121:y:2011:i:12:p:2802-2817} yields that the process 
\begin{align}
\left( Z_t := Y_{\Gamma_t} \right)_{t \leq T}
\end{align}
satisfies
\begin{align}
\left(Z_T, \sup_{u \leq T} Z_u \right) \sim \mathcal{M}_T,
\label{eq:model_one_marginal}
\end{align}
i.e. $Z$ is a Gamma subordinated diffusion-type process which calibrates to both, Vanilla and Barrier options.




\subsection{Diffusion-Type Model for Continuum of Maturities}

Assume $\left( \mathcal{M}_t \right)_{t \leq T}$ is given. Then define (assuming everything is well defined),
\begin{align}
V(t,x,m) := \int \left( x - y \right)^+ \mathcal{M}_{t}(\dd y, m).
\label{eq:V}
\end{align}

Several authors, including \citet[Theorem 3.6]{brunick2013}, \citet{Forde13} and \citet{Forde14}, consider diffusion-type processes of the form
\begin{align}
Z_t = Z_0 + \int_0^t \sigma(u,Z_u,M_u) \dd W_u, \qquad t \leq T.
\label{eq:diffusion_type_process_shreve}
\end{align}

It seems natural to try to choose $\sigma$ appropriately in order to match the marginals 
\begin{align*}
(Z_t, M_t) \sim \mathcal{M}_t \qquad \forall t \leq T.
\end{align*}
This problem has been looked at by
\citet{Forde13} and \citet{Forde14} who derive generalized forward Kolmogorov equations for the process $Z$ in \eqref{eq:diffusion_type_process_shreve} and $V$ from \eqref{eq:V}. 
They also formalize how to extend the Dupire formula to our setting, in particular they state sufficient conditions on $\sigma$ and $V$ for this \enquote{calibration} to work.

We finish this section by showing formally the intuition behind this generalized Dupire formula.
If we assume that the probability density function of $(Z_t,M_t)$, denoted by $p$, exists, then it is shown in Remark 7.2 of \citet{Forde13} that it satisfies the family of forward Kolmogorov equations:
\begin{align}
\frac{\partial p}{\partial t}(t,x,m) = \frac{1}{2} \frac{\partial^2}{\partial x^2} \Big( \sigma(t,x,m) p(t,x,m) \Big).
\end{align}

Then, following the arguments of \citet{Dup96} we obtain
\begin{align*}
\frac{\partial V}{\partial t}(t,x,m) = \frac{1}{2} \sigma^2(t,x,m) \frac{\partial^2 V}{\partial x^2}(t,x,m)
\end{align*}
and hence choose
\begin{align*}
\sigma^2(t,x,m) = \frac{2 \cdot \frac{\partial V}{\partial t}(t,x,m)}{\frac{\partial^2 V}{\partial x^2} (t,x,m) }
\end{align*}
with boundary condition
\begin{align*}
V(t,m,m) = 0
\end{align*}
in order to have 
\begin{align*}
p(t,x,m) = \frac{\mathcal{M}_t( \dd x, \dd m )}{\dd x \dd m}.
\end{align*}



==> up_and_out_puts.tex <==

\section{Up-and-out Put Options}

The following result is essentially a rephrasing of Proposition 7.2 of \citet{Forde13}.
Equation \eqref{eq:forward_equation_Up-and-out Put Options} is the forward equation for the down-and-out put option with boundary condition \eqref{eq:forward_equation_Up-and-out Put Options_boundary_condition}. 
Equation \eqref{eq:formula_up_and_out_put} provides explicit expressions for certain up-and-out put options given the decomposition of Theorem \ref{thm:Characterization Market Model - Multiple Maturity}.
\begin{Proposition}[Up-and-out Put Options]
\label{prop:Up-and-out Put Options}
Let $K>0$ and $B>X_0$. 
Then
\begin{subequations}
\begin{align}
&\E{ \left( K - X_t \right)^+ \indicator{ M_t < B } } - ( K - X_0 )^+ 
= \frac{1}{2} \cdot \E{ L^K_{ t \wedge H_B } } - ( K - B )^+ \cdot \Prob{ M_t \geq B }, \label{eq:forward_equation_Up-and-out Put Options} \\
&\E{ \left( B - X_t \right)^+ \indicator{ M_t < B } } = \E{ \left( B - X_t \right) \indicator{ M_t < B } } = B - X_0.
\label{eq:forward_equation_Up-and-out Put Options_boundary_condition}
\end{align}
\end{subequations}
Further we have,
\begin{align}
\E{ \left( K - X_{T_l} \right)^+ \indicator{ M_{T_l} < B_j } } = \mathfrak{p}^{B_j}_{l}(K) - ( K - B_j )^+ \cdot b_l(B_j) 
\label{eq:formula_up_and_out_put}
\end{align}
where we set (recalling $\mathfrak{c}^{B_j}_{l}$ from \eqref{eq:definition_identification_1M})
\begin{align}
\mathfrak{p}^{B_j}_{l}(K) &:= K - X_0 + \mathfrak{c}^{B_j}_{l}(K).
\end{align}
\end{Proposition}

\begin{proof}%[Proof of Proposition \ref{prop:Up-and-out Put Options}]
The first part of the claim is obtained by following the arguments in Proposition 7.2 of \citet{Forde13}. We report them for completeness.
Observe that by the \Ito-Tanaka formula
\begin{alignat*}{3}
& \left( K - X_t \right)^+ \indicator{ H_B > t } + ( K - B ) \indicator{ H_B \leq t } - \left( K - X_0 \right)^+ \\
=& \left( K - X_{t \wedge H_B} \right)^+ - \left( K - X_0 \right)^+ 
= -\int_{0}^{t \wedge H_B} \indicator{ X_u \leq K } \dd X_u + \frac{1}{2} L^K_{t \wedge H_B }
\end{alignat*}
and \eqref{eq:forward_equation_Up-and-out Put Options} follows by taking expectations.
As for \eqref{eq:forward_equation_Up-and-out Put Options_boundary_condition}, we note,
\begin{alignat*}{3}
X_0 = & && \E{ X_{ t \wedge H_B } } = \E{ X_{ t } \indicator{ M_t < B } } + B \Prob{ M_t \geq B } \\
= &-&& \E{ \left( B - X_t \right) \indicator{ M_t < B } } + B 
= -\E{ \left( B - X_t \right)^+ \indicator{ M_t < B } } + B.
\end{alignat*}
As for the second claim we observe
\begin{align*}
\frac{1}{2} \cdot \E{ L^K_{ t \wedge H_B } } = - ( X_0 - K )^+  +  \E{ \left( X_{t \wedge H_{B}} - K \right)^+ }
\end{align*}
and 
\begin{align*}
\E{ \left( X_{T_l \wedge H_{B_j}} - K \right)^+ } = \mathfrak{c}^{B_j}_{l}(K) 
\end{align*}
and hence \eqref{eq:formula_up_and_out_put} follows by plugging this into \eqref{eq:forward_equation_Up-and-out Put Options}.
\end{proof}

